Fast Policy Extragradient Methods for Competitive Games with Entropy Regularization

This paper investigates the problem of computing the equilibrium of competitive games, which is often modeled as a constrained saddle-point optimization problem with probability simplex constraints. Despite recent efforts in understanding the last-iterate convergence of extragradient methods in the unconstrained setting, the theoretical underpinnings of these methods in the constrained settings, especially those using multiplicative updates, remain highly inadequate, even when the objective function is bilinear. Motivated by the algorithmic role of entropy regularization in single-agent reinforcement learning and game theory, we develop provably efficient extragradient methods to find the quantal response equilibrium (QRE) -- which are solutions to zero-sum two-player matrix games with entropy regularization -- at a linear rate. The proposed algorithms can be implemented in a decentralized manner, where each player executes symmetric and multiplicative updates iteratively using its own payoff without observing the opponent's actions directly. In addition, by controlling the knob of entropy regularization, the proposed algorithms can locate an approximate Nash equilibrium of the unregularized matrix game at a sublinear rate without assuming the Nash equilibrium to be unique. Our methods also lead to efficient policy extragradient algorithms for solving (entropy-regularized) zero-sum Markov games at similar rates. All of our convergence rates are nearly dimension-free, which are independent of the size of the state and action spaces up to logarithm factors, highlighting the positive role of entropy regularization for accelerating convergence.

==> comparison.tex <==
\section{Comparison with existing results}
\paragraph{OMWU}
Existing analysis is focused on analyzing OMWU in the unregularized setting. \cite{rakhlin2013optimization} showed that the regret of OMWU is on the order of $O(1/t)$, while \cite{daskalakis2018last,wei2020linear} studied convergence properties of the last iterate. In particular, under the assumption that the Nash equilibrium is unique for the unregularized matrix game, \cite{daskalakis2018last} showed the asymptotic convergence of the last iterate to the unique equilibrium, and \cite{wei2020linear} showed the last iterate achieves a linear rate of convergence after an initial phase of sublinear convergence, yet the iteration complexity is not as rosy as it seems. In particular, \cite{wei2020linear} showed that the iteration complexity of achieving $\KL{{\zeta}^\star}{\zeta^{(t)}}\le \epsilon$ is
\[
	\min \left\{\frac{\log|\cA||\cB|}{\eta^2\iota^4C^2}\cdot\frac{1}{\epsilon},\quad \frac{\log|\cA||\cB|}{\eta^2\iota^4C^2}\cdot\frac{1}{\eta^2\xi^2} + \frac{1}{\eta^2\iota^3C^2\xi^2}\log \frac{\eta^2\xi^2}{\epsilon}\right\}
\]
where $C, \xi \in (0, \norm{A}_\infty)$ are problem-dependent constants and 
\[
	\iota = \min_{j\in {\rm supp}({\zeta}^\star)}\exp\prn{-\frac{\ln |\cA||\cB|}{\zeta^\star(j)}}.
\]
It is easily seen that $\iota^{-1} \ge |\cA||\cB|$ and can be even as large as $|\cA|^{|\cA|}|\cB|^{|\cB|}$ when $\zeta^\star = [\mu^\star, \nu^\star]$ are two uniform random policies. Therefore, the iteration complexity has a polynomial or even exponential dependency on the problem's dimensionality $|\cA|$, $|\cB|$.

\paragraph{OGDA} \cite{wei2020linear} also studied last-iterate convergence of OGDA for both matrix games and strongly-convex strongly-concave saddle point optimization problem. When applied to un-regularized matrix games, OGDA takes at most
\[
    O\prn{\frac{1}{\eta^2 C^2} \log \frac{1}{\epsilon}}
\]
iterations to achieve $\min_{\zeta^\star \text{is NE}} \norm{\zeta^\star - \zeta^{(t)}}_2^2 \le \epsilon$ \cite[Theorem 5, 8]{wei2020linear}.

In terms of the regularized problem, \citet[Theorem 6, 8]{wei2020linear} showed that OGDA takes
\[
    O\prn{\frac{1}{\eta^2 \tau^2} \log \frac{1}{\epsilon}}
\]
iterations to achieve $\norm{\best{\zeta} - \zeta^{(t)}}_2^2 \le \epsilon$, which is slower than our results by a factor of $1/\eta\tau$.
